Querying Multimodal Scientific Papers with AI: Practices and Preferences Across Blind, Low-Vision, and Sighted Scientists

Visual diagrams, figures, and tables are central to scientific papers, and convey information beyond what is captured in text. While blind or low-vision (BLV) scientists have traditionally relied on static alternative text to access figures in papers, the rise of artificial intelligence (AI) has made interactive question-answering (QA) a feasible paradigm for visual exploration; yet little is known about how scientists use visual QA in practice or how to improve its accessibility. In this work, we interview five BLV and five sighted scientists across different STEM fields to understand how they use two AI tools, ChatGPT and Gemini, to query multimodal scientific documents. Our findings characterize how scientists review multimodal content, including existing practices (along with accessibility workarounds) for engaging with visuals, and feedback on the suitability of AI-generated responses to multimodal queries. We further find that vague or incomplete image descriptions, as well as incorrect AI outputs more broadly, can cause both BLV and sighted scientists to abandon AI workflows. To support future research, we additionally contribute a dataset of 115 queries and responses from our participants' interactions with the AI tools for papers in their field. We close by discussing implications for AI-powered scientific QA systems, emphasizing considerations for access across abilities and domains.

==> longtable_with_category.tex <==
\begin{longtable}{p{0.8cm} p{3.5cm} p{0.8cm} p{1.2cm} p{1.2cm} p{3.5cm} p{3.5cm}}
\caption{Participant Queries and Paper Metadata} \label{tab:queries} \\
\toprule
\textbf{ID} & \textbf{Query} & \textbf{Category} & \textbf{Familiar/ Unfamiliar} & \textbf{Tool} & \textbf{Paper Title} & \textbf{Paper Link} \\ \midrule
\endfirsthead

\multicolumn{7}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\midrule
\textbf{ID} & \textbf{Query} & \textbf{Category} & \textbf{Familiar?} & \textbf{Tool} & \textbf{Paper Title} & \textbf{Paper Link} \\ \midrule
\endhead

% \midrule
% \multicolumn{7}{r}{{Continued on next page...}} \\
% \bottomrule
% \endfoot

\bottomrule
\endlastfoot
BLV1 & List and summarize all the figures in this research paper. Include the provided alt text description (if any) and the title/caption in the figure. & 2 & Familiar & ChatGPT & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
BLV1 & In figure 9, describe the type of chart and the chart itself. & 2 & Familiar & ChatGPT & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
BLV1 & go through each individual participant plotted and describe the individual trends. Try to estimate the percentages if not explicitly marked on the figure. & 2 & Familiar & ChatGPT & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
BLV1 & Give me an overview of Figure 3. Include the original caption and alt text (if any) and provide an overall description of the figure. & 2 & Familiar & Gemini & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
BLV1 & for each category of sounds, describe the corresponding haptic design based on the details in the figure and other text from the paper. & 3 & Familiar & Gemini & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
BLV1 & Give me an overview of this paper. Tell me what the contribution(s) are and an overall summary of the structure of the paper. & 1 & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
BLV1 & what's the stated cost of building this display? & 3 & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
BLV1 & In list item 3 that you mentioned, dive deeper into the technical details of how the pins are actuated and the modular design. & 3 & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
BLV1 & List the figures (if any) that illustrate the actuation mechanism/design. & 2 & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
BLV1 & Tell me about all the figures that illustrate how the actuation mechanism works in the tool described in this paper. Don't list figures that detail the fabrication process of how the researchers built the device, but do list the figures that describe how the actuation works. & 2 & Unfamiliar & ChatGPT & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
BLV1 & Describe how the actuation mechanism works using figure 6 and details included in section 4.3. How do the pins stay raised and how do they get lowered if there isn't an actuator for every pin as mentioned in other parts of the paper & 2 & Unfamiliar & ChatGPT & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
S1 & describe the main sealing methods tested in this paper and describe the main test conditions for the shaft seal & 3 & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & show a diagram & 4 & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & tell me about the shaft seal performance at high temperature and high compression & 3 & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & what was the shape of the relationship of leak rate vs pressure & 3 & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & tabulate figure 3 & 2 & Familiar & Gemini & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & my shaft diameter is 3" with differential pressure of 8 psi. What would my leak rate be in Standard L/min & 3 & Familiar & Gemini & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & any authors still alive and practicing & 4 & Familiar & Gemini & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
S1 & summarize the paper & 1 & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & How does tempering effect CTE? & 3 & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & How much residual austenite is in annealed 410 compared to H13 & 3 & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & would this paper be helpful for assessing the effect of annealing on 410 stainless? & 3 & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & tell me how this paper relates to the annealed cte of 410 stainless compared to full hard & 3 & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & what are the reciprocal lattice parameters of two carbides & 3 & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & in figure 6 list the major 2 theta peaks & 2 & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & what are they doing with the electro-chem setup & 3 & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S1 & what was the result and how did phase fraction drive them & 3 & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
S2 & Give me a summary of this paper & 1 & Familiar & Gemini & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
S2 & what are some future directions for this work & 4 & Familiar & Gemini & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
S2 & Give me a summary of this paper & 1 & Familiar & ChatGPT & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
S2 & tell me about figure 1 & 2 & Familiar & ChatGPT & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
S2 & give me a breakdown of each type of infection and frequencies for each course & 3 & Familiar & ChatGPT & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
S2 & Give me a summary of this paper as I am not familiar with it & 1 & Unfamiliar & ChatGPT & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
S2 & How many patients had proven vs probable infection? & 3 & Unfamiliar & ChatGPT & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
S2 & whats the breakdown of organism within the two groups? & 3 & Unfamiliar & ChatGPT & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
S2 & What are the breakdowns of type of fungal infection within the proven and probable categories of infection? & 3 & Unfamiliar & Gemini & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
S2 & Can you give me a summary of figure 2? & 2 & Unfamiliar & Gemini & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
S3 & Can you summarize the statistically significant outcomes from the fasting intervention & 3 & Familiar & Gemini & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
S3 & What was the size of the study and any other details of the population? & 3 & Familiar & Gemini & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
S3 & What are the specifics of the intervention? & 3 & Familiar & Gemini & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
S3 & what are the significant outcomes from this intervention & 3 & Familiar & ChatGPT & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
S3 & what is the most meangingful metric from table 2? & 2 & Familiar & ChatGPT & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
S3 & i'm interested in clinical data for plant polyphenols, does this study reference any clinical studies & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & can you share more about the specific clinical outcomes for curcumin & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & Are there specific mechanisms of action described that apply to all plant polyphenols discussed? & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & Are there any cancer studies mentioned? & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & does this paper differentiate between dietary sources of polyphenols and supplements and their difference in effectiveness? & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & can you dig into this further? Is there any data demonstrating dietary polyphenols with clinical outcomes & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & Are you sure this was a study of diet and not supplement/extract ? Blood pressure — RCTs and meta-analyses: Several RCTs and meta-analyses show dietary polyphenols (epicatechin, catechins, anthocyanins, quercetin) lower systolic and diastolic blood pressure (effects often dose-dependent; e.g., epicatechin minimum \textbackslash{}textasciitilde{}25 mg/day). & 3 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & in one table animal models given doxorubicin were summarized, can you tell me the outcomes in a simple summary? & 2 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
S3 & in table 7 what is the overall takeaway of resveratrol in animal models? & 2 & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
BLV2 & What conclusions do the authors come up with regarding screen vs text reading with a list of caveats included? & 3 & Unfamiliar & ChatGPT & A Comparison of Children’s Reading on Paper Versus Screen: A Meta-Analysis & \url{https://www.semanticscholar.org/paper/A-Comparison-of-Children%E2%80%99s-Reading-on-Paper-Versus-Furenes-Kucirkova/d3783034db2c17095e713a0a801d01a031fbe58f} \\
BLV2 & Please summarize the 1st flow chart in this document & 2 & Unfamiliar & Gemini & A Comparison of Children’s Reading on Paper Versus Screen: A Meta-Analysis & \url{https://www.semanticscholar.org/paper/A-Comparison-of-Children%E2%80%99s-Reading-on-Paper-Versus-Furenes-Kucirkova/d3783034db2c17095e713a0a801d01a031fbe58f} \\
BLV2 & It's unclear to me what is going on in figure one. Could you please provide a high level overview of the entire chart setup & 2 & Unfamiliar & Gemini & A Comparison of Children’s Reading on Paper Versus Screen: A Meta-Analysis & \url{https://www.semanticscholar.org/paper/A-Comparison-of-Children%E2%80%99s-Reading-on-Paper-Versus-Furenes-Kucirkova/d3783034db2c17095e713a0a801d01a031fbe58f} \\
BLV2 & Give me an overview of the background of author Rule from internet data including background on research with blind students such as in this article & 4 & Familiar & ChatGPT & Tactile Earth and Space Science Materials for Students with Visual Impairments: Contours, Craters, Asteroids, and Features of Mars & \url{https://www.tandfonline.com/doi/abs/10.5408/1.3651404} \\
BLV2 & Is there an image in the paper that would appear to show one of the Mars maps and if so what sort of information seems to be highlighted within the image & 2 & Familiar & ChatGPT & Tactile Earth and Space Science Materials for Students with Visual Impairments: Contours, Craters, Asteroids, and Features of Mars & \url{https://www.tandfonline.com/doi/abs/10.5408/1.3651404} \\
BLV2 & Using your knowledge reagrding Vallis Marineris and ideas of tactile graphics what would you suggest highlighting for understanding for blind students? Compare back to what the authors did with analysis of match percentage to your answer & 3 & Familiar & ChatGPT & Tactile Earth and Space Science Materials for Students with Visual Impairments: Contours, Craters, Asteroids, and Features of Mars & \url{https://www.tandfonline.com/doi/abs/10.5408/1.3651404} \\
BLV3 & Summarize the findings in this uploaded paper by Dutkiewicz et al, focus on the results, figures, diagrams, graphs, and images. If there are no visuals such as figures, diagrams, graphs, or images then do not hallucinate them. Keep the summary concise, include any math mentioned in the paper. & 1 & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
BLV3 & What was in figures 1a and 1b, and why did you mention the fourth bulletin point under 1. Carbonate Sequestration \textbackslash{}& Storage as you have in parenthesis that this is covering figures 1C and 1D yet mention 1B explain in concise details do not make up information & 2 & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
BLV3 & did you omit any other findings that others are reliant upon for their intrepetation? & 4 & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
BLV3 & use the visuals in the paper and make alt text for them, make sure you link the visual with the alt text so that a sighted person can verify the alt text, don't embed the alt text in the image, but produce it seperately & 2 & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
BLV3 & Figure 3 shows global visuals, add alt text to figure 3, make sure you include all information such as trend patterns, ledgers, axis units and scale, axis names, and title of the images, this is a global visual so use reference points to the continents that can be identified in the visual when you create the alt text, do not make up interpretations and do not add hallucinates. & 2 & Unfamiliar & Gemini & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
BLV3 & Identify and name the subduction zones, pure carbonate platforms, and paleo-coastlines in figure 3 and describe where they are at in comparison to the results. Do not make up coastlines, paleo-coastlines, pure carbonate platforms, and subduction zones. Parameterize the information to fit with figure 3. Turnicate jargon when possible, don’t hallucinate. & 2 & Unfamiliar & Gemini & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
BLV3 & Describe key finds in this pdf by Guy Munhoven, don’t hallucinate or make up results, don’t use information outside this paper to describe key finds. Add alt text to any visuals in the paper, make sure to include all details of these visuals such as global trends using geological names for features such as subduction zones, ridges, continents, shorelines, ocean basin, title all axises, give axis units, include graph titles, and ledger information, don’t make up figures or visuals & 1 & Familiar & Gemini & Model of Early Diagenesis in the Upper Sediment with Adaptable complexity – MEDUSA (v. 2): a time-dependent biogeochemical sediment module for Earth system models, process analysis and teaching & \url{https://www.researchgate.net/publication/352412122_Model_of_Early_Diagenesis_in_the_Upper_Sediment_with_Adaptable_complexity_-_MEDUSA_v_2_a_time-dependent_biogeochemical_sediment_module_for_Earth_system_models_process_analysis_and_teaching} \\
S4 & hey gemini, tell me about this paper - focus on what are the findings and what experiment paradigm and analysis were used. & 1 & Unfamiliar & Gemini & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & what is the key plot or figure that conveys the main finding of the paper & 2 & Unfamiliar & Gemini & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & could you summarize this paper to me focusing on the hypothesis first, methods used to test the hypothesis and key findings & 1 & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & give me some intuitions for what avalanche analysis does and when it can be used. why is it suitable to apply here? & 3 & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & what are the main plots that convey the main findings of this paper? & 2 & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & help me understand figure 1J. what is PL ? & 2 & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & could you interpret Fig 1J for me? & 2 & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
S4 & in this paper, when they did factor analysis, did they report the dimensionality trends of readout population with learning? & 3 & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & how is shared dimensionality different from overall dimensionality of readouts? & 3 & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & yes please & 4 & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & Could you point me to the key plots in the paper that convey the main findings? & 2 & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & hey gemini, could you explain how the private and shared variance analysis could help us understand neural learning? & 3 & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & did they look at overall dimensionality trends of readouts with learning? & 3 & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & in neuroscience, overall dimensionality would be the degree of freedom that neural activity explores not the number of neurons themselves. With this context, could you tell me if the paper looked at overall readout dimensionality trends. How does Factor analysis separate variance ? & 3 & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
S4 & what are the key plots that convey the main findings of the paper? help me understand them & 2 & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
BLV4 & Can you give me a concise overview of this paper, especially methods and key findings? & 1 & Unfamiliar & Gemini & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
BLV4 & Can you elaborate on the study design a bit more? Specifically, what do you mean by "minimally-guided meditation sessions"? & 3 & Unfamiliar & Gemini & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
BLV4 & Please describe the pilot study from start to finish. In particular, I would like to learn more about how the research team determined possible body placement(s) for the device. & 3 & Unfamiliar & ChatGPT & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
BLV4 & I would now like a timeline-style summary of the main study itself. And if applicable, I would like you to note where each stage of the pilot studies was instrumental in crafting and refining the main study protocol. & 3 & Unfamiliar & ChatGPT & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
BLV4 & Can you please describe in detail the figures of this paper, what they aimed to show the reader, and why they were helpful in illustrating the authors' findings? & 2 & Familiar & Gemini & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
BLV4 & No, I want to know what specific plots were used for each of these figures & 2 & Familiar & Gemini & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
BLV4 & In Figure 3, each of the two plots have short, horizontal lines below each of the vertical lines for each condition. They also appear in different colors. What do these short, horizontal lines mean? Are they significant to understanding these plots and this figure? & 2 & Familiar & ChatGPT & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
BLV4 & Why did the authors decide to use the means of Likert scale data in their visualizations? Do you think that this was the strongest way to visualize this data, or could there have been other measures that more appropriately captured insights from the Likert scale data? & 3 & Familiar & ChatGPT & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
BLV5 & I am uploading a paper in PDF format that I got from ArXiV. Tell me how this paper relates to my work in aligning multimodal embeddings with neural activity. & 3 & Familiar & ChatGPT & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
BLV5 & I am not very familiar with DIONv3 models. Why do the authors used those specifically and how would that be compared with my current ViT\textbackslash{}_l\textbackslash{}_16 backbones. & 3 & Familiar & ChatGPT & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
BLV5 & Based on the attached pdf. Explain to me how it relates with my current research on brain alignment of multimodal models. & 3 & Familiar & Gemini & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
BLV5 & Describe for me this image from the paper: & 2 & Familiar & Gemini & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
BLV5 & I am uploading a 2021 neurIPS paper. I want you to: 1. extract the full text form the PDF. 2. carefully parce through the. 3. genrate a blind-friendly explanation on how this paper relates with my work. & 1 & Unfamiliar & Gemini & Attention Bottlenecks for Multimodal Fusion. & \url{https://arxiv.org/abs/2107.00135} \\
BLV5 & this is the file now & 4 & Unfamiliar & Gemini & Attention Bottlenecks for Multimodal Fusion. & \url{https://arxiv.org/abs/2107.00135} \\
BLV5 & generate a blind friendly, math and code focused of the figures of the paper. Explain to me how they were genrated, how would I present them on a lab meeting and how I could generate similar visuals & 2 & Unfamiliar & Gemini & Attention Bottlenecks for Multimodal Fusion. & \url{https://arxiv.org/abs/2107.00135} \\
S5 & Can you please summarize the different evaluation metrics of this benchmark? & 3 & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & Is the model querying different when measuring with coverage or average precision? & 3 & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & Is there any explicit suggestions of wanting coverage between runs? And what is the temperature? & 3 & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & What was the prompt for the agent fro the multiple choice example? & 3 & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & What is the text in Figure 19? & 2 & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & How about the prompt for analysis generation? & 3 & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & What are the prompts used for the agentic analysis generation? & 3 & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & What are examples of the different decision points and possible analysis decisions? & 3 & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & In the appendix, it talks about column pointer nodes where do those come from in the data? & 3 & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & In figure 4, what kinds of models do better and what do worse? & 2 & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & What decision points have the biggest precision range for model capabilities? & 2 & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
S5 & Who validates the validators? & 1 & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & What were some participant quotes related to criteria drift? & 3 & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & But what does it mean if criteria are always updating? How do they argue we can formulate correctness or evaluations? & 3 & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & What related work do they use to justify or support this criteria drift finding? & 3 & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & How does this differ from generic human in the loop model updating? & 3 & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & Is there anything discussed in the text that isn't shown in figure 1 (or vice versa) & 2 & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & Hmmm, instead of conceptual differences, I mean for the specific textual explanation of the EVALGEN Evaluation pipeline method, are there specific difference between the methods as described in the text and the Figure 1b diagram & 2 & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & In figure 2 part d, which part of figure 1 does it relate to? & 2 & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & In Table 1, Between the medical and product pipeline, what are important takeaways? & 2 & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
S5 & What are the downsides of this approach? & 3 & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\end{longtable}

==> queries_table.tex <==
BLV1 & List and summarize all the figures in this research paper. Include the provided alt text description (if any) and the title/caption in the figure. & Familiar & ChatGPT & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
\hline
BLV1 & In figure 9, describe the type of chart and the chart itself. & Familiar & ChatGPT & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
\hline
BLV1 & go through each individual participant plotted and describe the individual trends. Try to estimate the percentages if not explicitly marked on the figure. & Familiar & ChatGPT & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
\hline
BLV1 & Give me an overview of Figure 3. Include the original caption and alt text (if any) and provide an overall description of the figure. & Familiar & Gemini & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
\hline
BLV1 & for each category of sounds, describe the corresponding haptic design based on the details in the figure and other text from the paper. & Familiar & Gemini & Typing Haptically: Towards Enabling Non-auditory Smartphone Text Entry with Haptic Feedback for Blind and Low Vision Users & \url{http://dl.acm.org/doi/10.1145/3746059.3747801} \\
\hline
BLV1 & Give me an overview of this paper. Tell me what the contribution(s) are and an overall summary of the structure of the paper. & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
\hline
BLV1 & what's the stated cost of building this display? & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
\hline
BLV1 & In list item 3 that you mentioned, dive deeper into the technical details of how the pins are actuated and the modular design. & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
\hline
BLV1 & List the figures (if any) that illustrate the actuation mechanism/design. & Unfamiliar & Gemini & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
\hline
BLV1 & Tell me about all the figures that illustrate how the actuation mechanism works in the tool described in this paper. Don't list figures that detail the fabrication process of how the researchers built the device, but do list the figures that describe how the actuation works. & Unfamiliar & ChatGPT & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
\hline
BLV1 & Describe how the actuation mechanism works using figure 6 and details included in section 4.3. How do the pins stay raised and how do they get lowered if there isn't an actuator for every pin as mentioned in other parts of the paper & Unfamiliar & ChatGPT & MagnePins: A Modular, Affordable, and DIY Refreshable Braille and Tactile Display & \url{https://dl.acm.org/doi/10.1145/3746059.3747692} \\
\hline
S1 & describe the main sealing methods tested in this paper and describe the main test conditions for the shaft seal & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & show a diagram & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & tell me about the shaft seal performance at high temperature and high compression & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & what was the shape of the relationship of leak rate vs pressure & Familiar & ChatGPT & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & tabulate figure 3 & Familiar & Gemini & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & my shaft diameter is 3" with differential pressure of 8 psi. What would my leak rate be in Standard L/min & Familiar & Gemini & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & any authors still alive and practicing  & Familiar & Gemini & High Temperature Braided Rope Seals for Static Sealing Applications & \url{https://arc.aiaa.org/doi/10.2514/2.5219} \\
\hline
S1 & summarize the paper & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & How does tempering effect CTE? & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & How much residual austenite is in annealed 410 compared to H13 & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & would this paper be helpful for assessing the effect of annealing on 410 stainless? & Unfamiliar & ChatGPT & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & tell me how this paper relates to the annealed cte of 410 stainless compared to full hard & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & what are the reciprocal lattice parameters of two carbides  & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & in figure 6 list the major 2 theta peaks & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & what are they doing with the electro-chem setup & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S1 & what was the result and how did phase fraction drive them & Unfamiliar & Gemini & Effect of Heat Treatment on Thermal Expansion Behavior and Corrosion Resistance of Martensitic Stainless Steel Manufactured by Submerged Arc Welding & \url{https://www.semanticscholar.org/paper/Effect-of-Heat-Treatment-on-Thermal-Expansion-and-Wang/3a0fa050f580d71f374f175bfddf57942a229029} \\
\hline
S2 & Give me a summary of this paper & Familiar & Gemini & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
\hline
S2 & what are some future directions for this work & Familiar & Gemini & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
\hline
S2 & Give me a summary of this paper & Familiar & ChatGPT & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
\hline
S2 & tell me about figure 1 & Familiar & ChatGPT & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
\hline
S2 & give me a breakdown of each type of infection and frequencies for each course & Familiar & ChatGPT & Infectious events in pediatric patients with acute lymphoblastic leukemia/lymphoma undergoing evaluation for fever without severe neutropenia & \url{https://pubmed.ncbi.nlm.nih.gov/36238979/} \\
\hline
S2 & Give me a summary of this paper as I am not familiar with it & Unfamiliar & ChatGPT & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
\hline
S2 & How many patients had proven vs probable infection? & Unfamiliar & ChatGPT & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
\hline
S2 & whats the breakdown of organism within the two groups? & Unfamiliar & ChatGPT & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
\hline
S2 & What are the breakdowns of type of fungal infection within the proven and probable categories of infection? & Unfamiliar & Gemini & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
\hline
S2 & Can you give me a summary of figure 2? & Unfamiliar & Gemini & Invasive fungal diseases impact on outcome of childhood ALL – an analysis of the international trial AIEOP-BFM ALL 2009 & \url{https://pubmed.ncbi.nlm.nih.gov/36509893/} \\
\hline
S3 & Can you summarize the statistically significant outcomes from the fasting intervention & Familiar & Gemini & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
\hline
S3 & What was the size of the study and any other details of the population? & Familiar & Gemini & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
\hline
S3 & What are the specifics of the intervention? & Familiar & Gemini & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
\hline
S3 & what are the significant outcomes from this intervention & Familiar & ChatGPT & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
\hline
S3 & what is the most meangingful metric from table 2? & Familiar & ChatGPT & Fasting mimicking diet during neo-adjuvant chemotherapy in breast cancer patients: a randomized controlled trial study & \url{https://pubmed.ncbi.nlm.nih.gov/39703333/} \\
\hline
S3 & i'm interested in clinical data for plant polyphenols, does this study reference any clinical studies & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & can you share more about the specific clinical outcomes for curcumin & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & Are there specific mechanisms of action described that apply to all plant polyphenols discussed? & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & Are there any cancer studies mentioned? & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & does this paper differentiate between dietary sources of polyphenols and supplements and their difference in effectiveness? & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & can you dig into this further? Is there any data demonstrating dietary polyphenols with clinical outcomes & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & Are you sure this was a study of diet and not supplement/extract ? Blood pressure — RCTs and meta-analyses: Several RCTs and meta-analyses show dietary polyphenols (epicatechin, catechins, anthocyanins, quercetin) lower systolic and diastolic blood pressure (effects often dose-dependent; e.g., epicatechin minimum \textbackslash{}textasciitilde{}25 mg/day). & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & in one table animal models given doxorubicin were summarized, can you tell me the outcomes in a simple summary? & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
S3 & in table 7 what is the overall takeaway of resveratrol in animal models? & Unfamiliar & Gemini & Plant Polyphenols as Heart's Best Friends: From Health Properties, to Cellular Effects, to Molecular Mechanisms of Action & \url{https://pubmed.ncbi.nlm.nih.gov/39940685/} \\
\hline
BLV2 & What conclusions do the authors come up with regarding screen vs text reading with a list of caveats included? & Unfamiliar & ChatGPT & A Comparison of Children’s Reading on Paper Versus Screen: A Meta-Analysis & \url{https://www.semanticscholar.org/paper/A-Comparison-of-Children%E2%80%99s-Reading-on-Paper-Versus-Furenes-Kucirkova/d3783034db2c17095e713a0a801d01a031fbe58f} \\
\hline
BLV2 & Please summarize the 1st flow chart in this document & Unfamiliar & Gemini & A Comparison of Children’s Reading on Paper Versus Screen: A Meta-Analysis & \url{https://www.semanticscholar.org/paper/A-Comparison-of-Children%E2%80%99s-Reading-on-Paper-Versus-Furenes-Kucirkova/d3783034db2c17095e713a0a801d01a031fbe58f} \\
\hline
BLV2 & It's unclear to me what is going on in figure one. Could you please provide a high level overview of the entire chart setup & Unfamiliar & Gemini & A Comparison of Children’s Reading on Paper Versus Screen: A Meta-Analysis & \url{https://www.semanticscholar.org/paper/A-Comparison-of-Children%E2%80%99s-Reading-on-Paper-Versus-Furenes-Kucirkova/d3783034db2c17095e713a0a801d01a031fbe58f} \\
\hline
BLV2 & Give me an overview of the background of author Rule from internet data including background on research with blind students such as in this article & Familiar & ChatGPT & Tactile Earth and Space Science Materials for Students with Visual Impairments: Contours, Craters, Asteroids, and Features of Mars & \url{https://www.tandfonline.com/doi/abs/10.5408/1.3651404} \\
\hline
BLV2 & Is there an image in the paper that would appear to show one of the Mars maps and if so what sort of information seems to be highlighted within the image & Familiar & ChatGPT & Tactile Earth and Space Science Materials for Students with Visual Impairments: Contours, Craters, Asteroids, and Features of Mars & \url{https://www.tandfonline.com/doi/abs/10.5408/1.3651404} \\
\hline
BLV2 & Using your knowledge reagrding Vallis Marineris and ideas of tactile graphics what would you suggest highlighting for understanding for blind students? Compare back to what the authors did with analysis of match percentage to your answer & Familiar & ChatGPT & Tactile Earth and Space Science Materials for Students with Visual Impairments: Contours, Craters, Asteroids, and Features of Mars & \url{https://www.tandfonline.com/doi/abs/10.5408/1.3651404} \\
\hline
BLV3 & Summarize the findings in this uploaded paper by Dutkiewicz et al, focus on the results, figures, diagrams, graphs, and images. If there are no visuals such as figures, diagrams, graphs, or images then do not hallucinate them. Keep the summary concise, include any math mentioned in the paper. & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
\hline
BLV3 & What was in figures 1a and 1b, and why did you mention the fourth bulletin point under 1. Carbonate Sequestration \textbackslash{}& Storage as you have in parenthesis that this is covering figures 1C and 1D yet mention 1B explain in concise details do not make up information & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
\hline
BLV3 & did you omit any other findings that others are reliant upon for their intrepetation? & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
\hline
BLV3 & use the visuals in the paper and make alt text for them, make sure you link the visual with the alt text so that a sighted person can verify the alt text, don't embed the alt text in the image, but produce it seperately & Unfamiliar & ChatGPT & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
\hline
BLV3 & Figure 3 shows global visuals, add alt text to figure 3, make sure you include all information such as trend patterns, ledgers, axis units and scale, axis names, and title of the images, this is a global visual so use reference points to the continents that can be identified in the visual when you create the alt text, do not make up interpretations and do not add hallucinates. & Unfamiliar & Gemini & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
\hline
BLV3 & Identify and name the subduction zones, pure carbonate platforms, and paleo-coastlines in figure 3 and describe where they are at in comparison to the results. Do not make up coastlines, paleo-coastlines, pure carbonate platforms, and subduction zones. Parameterize the information to fit with figure 3. Turnicate jargon when possible, don’t hallucinate. & Unfamiliar & Gemini & Sequestration and subduction of deep-sea carbonate in the global ocean since the Early Cretaceous & \url{https://pubs.geoscienceworld.org/gsa/geology/article-abstract/47/1/91/567642/Sequestration-and-subduction-of-deep-sea-carbonate} \\
\hline
BLV3 & Describe key finds in this pdf by Guy Munhoven, don’t hallucinate or make up results, don’t use information outside this paper to describe key finds. Add alt text to any visuals in the paper, make sure to include all details of these visuals such as global trends using geological names for features such as subduction zones, ridges, continents, shorelines, ocean basin, title all axises, give axis units, include graph titles, and ledger information, don’t make up figures or visuals & Familiar & Gemini & Model of Early Diagenesis in the Upper Sediment with Adaptable complexity – MEDUSA (v. 2): a time-dependent biogeochemical sediment module for Earth system models, process analysis and teaching & \url{https://www.researchgate.net/publication/352412122_Model_of_Early_Diagenesis_in_the_Upper_Sediment_with_Adaptable_complexity_-_MEDUSA_v_2_a_time-dependent_biogeochemical_sediment_module_for_Earth_system_models_process_analysis_and_teaching} \\
\hline
S4 & hey gemini, tell me about this paper - focus on what are the findings and what experiment paradigm and analysis were used. & Unfamiliar & Gemini & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & what is the key plot or figure that conveys the main finding of the paper & Unfamiliar & Gemini & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & could you summarize this paper to me focusing on the hypothesis first, methods used to test the hypothesis and key findings & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & give me some intuitions for what avalanche analysis does and when it can be used. why is it suitable to apply here? & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & what are the main plots that convey the main findings of this paper? & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & help me understand figure 1J. what is PL ? & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & could you interpret Fig 1J for me? & Unfamiliar & ChatGPT & Low-dimensional criticality embedded in high-dimensional awake brain dynamics & \url{https://pubmed.ncbi.nlm.nih.gov/38669340/} \\
\hline
S4 & in this paper, when they did factor analysis, did they report the dimensionality trends of readout population with learning? & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & how is shared dimensionality different from overall dimensionality of readouts? & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & yes please & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & Could you point me to the key plots in the paper that convey the main findings? & Familiar & ChatGPT & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & hey gemini, could you explain how the private and shared variance analysis could help us understand neural learning? & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & did they look at overall dimensionality trends of readouts with learning? & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & in neuroscience, overall dimensionality would be the degree of freedom that neural activity explores not the number of neurons themselves. With this context, could you tell me if the paper looked at overall readout dimensionality trends. How does Factor analysis separate variance ? & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
S4 & what are the key plots that convey the main findings of the paper? help me understand them  & Familiar & Gemini & Emergence of Coordinated Neural Dynamics Underlies Neuroprosthetic Learning and Skillful Control & \url{https://pubmed.ncbi.nlm.nih.gov/28190641/} \\
\hline
BLV4 & Can you give me a concise overview of this paper, especially methods and key findings? & Unfamiliar & Gemini & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
\hline
BLV4 & Can you elaborate on the study design a bit more? Specifically, what do you mean by "minimally-guided meditation sessions"? & Unfamiliar & Gemini & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
\hline
BLV4 & Please describe the pilot study from start to finish. In particular, I would like to learn more about how the research team determined possible body placement(s) for the device. & Unfamiliar & ChatGPT & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
\hline
BLV4 & I would now like a timeline-style summary of the main study itself. And if applicable, I would like you to note where each stage of the pilot studies was instrumental in crafting and refining the main study protocol. & Unfamiliar & ChatGPT & Somaesthetic Meditation Wearable: Exploring the Effect of Targeted Warmth Technology on Meditators’ Experiences & \url{https://dl.acm.org/doi/10.1145/3613904.3642557} \\
\hline
BLV4 & Can you please describe in detail the figures of this paper, what they aimed to show the reader, and why they were helpful in illustrating the authors' findings? & Familiar & Gemini & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
\hline
BLV4 & No, I want to know what specific plots were used for each of these figures & Familiar & Gemini & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
\hline
BLV4 & In Figure 3, each of the two plots have short, horizontal lines below each of the vertical lines for each condition. They also appear in different colors. What do these short, horizontal lines mean? Are they significant to understanding these plots and this figure? & Familiar & ChatGPT & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
\hline
BLV4 & Why did the authors decide to use the means of Likert scale data in their visualizations? Do you think that this was the strongest way to visualize this data, or could there have been other measures that more appropriately captured insights from the Likert scale data? & Familiar & ChatGPT & One vs. Many: Comprehending Accurate Information from Multiple Erroneous and Inconsistent AI Generations & \url{https://dl.acm.org/doi/10.1145/3630106.3662681} \\
\hline
BLV5 & I am uploading a paper in PDF format that I got from ArXiV. Tell me how this paper relates to my work in aligning multimodal embeddings with neural activity. & Familiar & ChatGPT & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
\hline
BLV5 & I am not very familiar with DIONv3 models. Why do the authors used those specifically and how would that be compared with my current ViT\textbackslash{}_l\textbackslash{}_16 backbones. & Familiar & ChatGPT & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
\hline
BLV5 & Based on the attached pdf. Explain to me how it relates with my current research on brain alignment of multimodal models. & Familiar  & Gemini & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
\hline
BLV5 & Describe for me this image from the paper: & Familiar  & Gemini & Disentangling the Factors of Convergence between Brains and Computer Vision Models & \url{https://arxiv.org/abs/2508.18226} \\
\hline
BLV5 & I am uploading a 2021 neurIPS paper. I want you to: 1. extract the full text form the PDF. 2. carefully parce through the. 3. genrate a blind-friendly explanation on how this paper relates with my work. & Unfamiliar & Gemini & Attention Bottlenecks for Multimodal Fusion. & \url{https://arxiv.org/abs/2107.00135} \\
\hline
BLV5 & this is the file now & Unfamiliar & Gemini & Attention Bottlenecks for Multimodal Fusion. & \url{https://arxiv.org/abs/2107.00135} \\
\hline
BLV5 & generate a blind friendly, math and code focused of the figures of the paper. Explain to me how they were genrated, how would I present them on a lab meeting and how I could generate similar visuals & Unfamiliar & Gemini & Attention Bottlenecks for Multimodal Fusion. & \url{https://arxiv.org/abs/2107.00135} \\
\hline
S5 & Can you please summarize the different evaluation metrics of this benchmark? & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & Is the model querying different when measuring with coverage or average precision? & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & Is there any explicit suggestions of wanting coverage between runs? And what is the temperature? & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & What was the prompt for the agent fro the multiple choice example? & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & What is the text in Figure 19? & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & How about the prompt for analysis generation? & Familiar & Gemini & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & What are the prompts used for the agentic analysis generation? & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & What are examples of the different decision points and possible analysis decisions? & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & In the appendix, it talks about column pointer nodes where do those come from in the data? & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & In figure 4, what kinds of models do better and what do worse? & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & What decision points have the biggest precision range for model capabilities? & Familiar & ChatGPT & BLADE: Benchmarking Language Model Agents for Data-Driven Science & \url{https://arxiv.org/abs/2408.09667} \\
\hline
S5 & Who validates the validators? & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & What were some participant quotes related to criteria drift? & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & But what does it mean if criteria are always updating? How do they argue we can formulate correctness or evaluations? & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & What related work do they use to justify or support this criteria drift finding? & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & How does this differ from generic human in the loop model updating? & Unfamiliar & Gemini & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & Is there anything discussed in the text that isn't shown in figure 1 (or vice versa) & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & Hmmm, instead of conceptual differences, I mean for the specific textual explanation of the EVALGEN Evaluation pipeline method, are there specific difference between the methods as described in the text and the Figure 1b diagram & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & In figure 2 part d, which part of figure 1 does it relate to? & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & In Table 1, Between the medical and product pipeline, what are important takeaways? & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\
\hline
S5 & What are the downsides of this approach? & Unfamiliar & ChatGPT & Who Validates the Validators? Aligning LLM-Assisted Evaluation of LLM Outputs with Human Preferences & \url{https://arxiv.org/abs/2404.12272} \\

